Robust Transductive Few-shot Learning via Joint Message Passing and Prototype-based Soft-label Propagation

Few-shot learning (FSL) aims to develop a learning model with the ability to generalize to new classes using a few support samples. For transductive FSL tasks, prototype learning and label propagation methods are commonly employed. Prototype methods generally first learn the representative prototypes from the support set and then determine the labels of queries based on the metric between query samples and prototypes. Label propagation methods try to propagate the labels of support samples on the constructed graph encoding the relationships between both support and query samples. This paper aims to integrate these two principles together and develop an efficient and robust transductive FSL approach, termed Prototype-based Soft-label Propagation (PSLP). Specifically, we first estimate the soft-label presentation for each query sample by leveraging prototypes. Then, we conduct soft-label propagation on our learned query-support graph. Both steps are conducted progressively to boost their respective performance. Moreover, to learn effective prototypes for soft-label estimation as well as the desirable query-support graph for soft-label propagation, we design a new joint message passing scheme to learn sample presentation and relational graph jointly. Our PSLP method is parameter-free and can be implemented very efficiently. On four popular datasets, our method achieves competitive results on both balanced and imbalanced settings compared to the state-of-the-art methods. The code will be released upon acceptance.

==> sec/3_old.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{img/Network.jpg}
    \caption{The process of the proposed method. First, we obtain the support and query samples features by the feature extractor. Then, all samples are feed into multi-order graph convolution for feature mapping, so that similar nodes are closer in the feature space. Then, we use the mapped features to construct a graph and use label propagation to alternately update the labels and prototypes, and output the prediction results.}
    \label{fig:network}
\end{figure*}

\section{Method}

In this section, we firstly introduce the task definition of transductive few-shot learning .
% Existing feature embedding methods often require parameter learning or subspace learning during testing, thereby impeding the inference speed.
Then, we present the method of Multi-order Graph Convolution (MGC) for feature embedding to enhance feature representation capability.
% It is noteworthy that this method generates feature embeddings based on features extracted by the backbone network and is parameter-free, making it compatible with most transductive few-shot classifiers.
Next, we introduce Fast Iterative Label Propagation (FILP), which utilizes all samples for label propagation and alternately updates prototypes and label matrix. We employ the label matrix of last iteration as the prediction result. Finally, we analyze the time complexity of the method. The diagram of our proposed approach is shown in Fig.\ref{fig:network}.

\subsection{Problem Formulation}
Under the few-shot scenario, let us assume that we have a large labeled base dataset $\mathcal{D}_{base} = {\{(\boldsymbol{x}^b_i,y^b_i)\}}_{i=1}^{n_{base}}$ with $C_{base}$ classes, where $n_{base}$ denotes the number of base class samples, and $\boldsymbol{x}_i^b$ and $y_i^b$ represent the sample features extracted by the backbone network $f_\theta$ and their corresponding labels, respectively. During the training phase, we training of $f_\theta$ on $\mathcal{D}_{base}$ with the supervision of labels. We are provided with another dataset of novel classes $\mathcal{D}_{novel} = {\{(\boldsymbol{x}_i,y_i)\}}_{i=1}^{n_{novel}}$ for evaluating classification performance. Here, the novel class labels $y_i$ are categories that the network has never encountered before, and satisfy $C_{novel}\cap C_{base} = \emptyset$.

During the inference phase, for an $N$-way $K$-shot task, we randomly sample support set $\mathcal{S} = {\{(\boldsymbol{x}^s_i,y^s_i)\}}_{i=1}^{NK} $ and query set $\mathcal{Q} = {\{\boldsymbol{x}^q_i\}}_{i=1}^{M} $ from $\mathcal{D}_{novel}$ to construct multiple tasks, indicating that the support set contains $N$ unseen categories, each with $K$ labeled samples, and the $M$ samples in the query set all belong to these $N$ categories. We focus on the transductive setting, where we employ $f_\theta$ to extract features and simultaneously utilize all samples from $\mathcal{S}$ and $\mathcal{Q}$, and predict labels  of the samples in $\mathcal{Q}$.

\subsection{Graph Message Propagation}
% The backbone network $f_\theta$ used for extracting features of test samples is learned from $\mathcal{D}_{base}$. However, it often fails to provide accurate feature representations when confronted with unseen classes in $\mathcal{D}_{novel}$.
To enhance the quality of feature representation, and get a it is necessary to map the sample features from the support set and query set.
% Previous methods often introduced a large number of learnable parameters at this step [hubs], or employed test-time learning through subspace learning [ease], severely affecting the inference speed and rendering them unsuitable for real-world deployment. To address this issue,
Firstly, we establish two primary objectives in designing the feature mapping process. One is to bring the features of query samples from the same class closer to the features of support samples of that class. The other is to fully leverage both query and support samples to better construct global connections between samples.
% The former contributes to enhancing the similarity of features among samples of the same class and the distinctiveness among samples of different classes, while the latter aids in constructing a reliable graph structure to facilitate subsequent label propagation.
Simultaneously, we argue that the process of feature mapping should not excessively consume inference time, thus ensuring the method's reliability in real-world applications. Therefore, we draw inspiration from \cite{agc} and propose a parameter-free multi-order graph convolution (MGC).
We apply low-pass filtering graph convolution to the features of support and query samples. Specifically, we first concatenate the features of support samples and query samples:
\begin{equation}
\label{eq:featureconcat}
    X = \mathrm{Concat}([(\boldsymbol{x}^s_1,\cdots,\boldsymbol{x}^s_{NK}],[(\boldsymbol{x}^q_1,\cdots,\boldsymbol{x}^q_M])
\end{equation}
Subsequently, we construct the similarity matrix $A = \mathrm{exp}(-\lambda\|\boldsymbol{x}_i-\boldsymbol{x}_j\|^2_2)$ and compute its degree matrix $D = \mathrm{diag}(\sum{_j^T}a_{ij})$, where $T = NK+M$ represents the total number of samples, and $\lambda$ is a hyperparameter. We obtain the symmetrically regularized graph Laplacian matrix as follows:
\begin{equation}
\label{eq:laplasi}
    L = I-D^{-\frac{1}{2}}AD^{-\frac{1}{2}} \in \mathbb{R}^{T\times T}
\end{equation}
Subsequently, the process of applying low-pass filtering graph convolution can be represented as:
\begin{equation}
\label{eq:featureproject1}
 \bar{X} = GX = (I-\frac{1}{2}L)X
\end{equation}
where, $G$ represents the low-pass filtering kernel, $\bar{X}$ denotes the convolved features, and $I$ signifies the identity matrix. Based on the assumption that adjacent nodes are likely to belong to the same category, performing graph convolution using Eq.\ref{eq:featureproject1} is equivalent to aggregating features from 1-hop neighboring nodes, allowing adjacent nodes to acquire more similar features through dense connections \cite{agc} and facilitating subsequent label propagation.

% Based on the assumption that adjacent nodes are likely to belong to the same category, applying this low-pass graph convolution to the features of support and query samples can bring features of the same category closer.

However, Eq.\ref{eq:featureproject1} does not fully leverage long-distance path correlations in the graph. To better capture the global graph structure and enhance the robustness of the structure, we apply a multi-order graph convolution kernel. The $k$-order graph convolution is defined as:
\begin{equation}
\label{eq:featureprojectK}
\bar{X} = G'X = (I-\frac{1}{2}L)^kX
\end{equation}
% K-th order graph convolution is equivalent to aggregating features from one's $k$-hop neighboring nodes, utilizing cross-sample correlations to construct a more robust graph structure.
MGC aggregates and maps features from the $k$-hop neighbors of samples. In terms of features, similar samples obtain more similar features; in terms of structure, samples construct a more robust graph structure by aggregating global correlations. Additionally, since MGC is parameter-free, it optimizes the original feature mapping at a very fast speed.

\subsection{Fast Iterative Label Propagation}

A considerable number of work has applied label propagation on data manifolds \cite{tpn,ilpc,am,epnet} to the task of transductive few-shot learning. However, these efforts face several main challenges. Firstly, it is difficult to iteratively optimizing the propagation results. Secondly, they fail to correct the biased distribution of support samples. Thirdly, handling imbalances in the number of query samples across different classes is challenging. Some approaches attempt to introduce a large number of learnable parameters \cite{am} and design complex optimization objectives \cite{protolp,ilpc}, resulting in network convergence issues. Thus, we propose a Fast Iterative Label Propagation (FILP) to optimize prototype and label matrix alternatively. We treat all samples as the source of propagation and simultaneously propagate of label propagation. So, FILP can adjusts the strength of label propagation for each class based on one-hot labels of support samples and pseudo-controls of query samples. Subsequently, we update prototypes based on the propagation results and recompute pseudo-labels for query samples. As FILP is parameter-free and only requires prototype updates, a few iterations are sufficient to obtain the label matrix for the prediction result.

Specifically, we first construct a similarity matrix $\bar{A} = \mathrm{exp}(-\lambda\|\bar{\boldsymbol{x}}_i-
\bar{\boldsymbol{x}}_j\|^2_2)$ based on the mapped features obtained by MGC. Since MGC has already established long-distance relationships, here we only retain the first $v$ neighbor for each sample:
\begin{equation}
\label{eq:sparselink}
\bar{a}_{ij} = 
\begin{cases}
\bar{a}_{ij} &\bar{a}_{ij}\in \mathrm{topv}(\bar{\boldsymbol{a}}_i)\\
 0& \mathrm{otherwise}
\end{cases}
\end{equation}
In label propagation, the relationship of nodes with themselves is not considered:
\begin{equation}
\label{eq:diag}
    \tilde{A} = \bar{A} - \mathrm{diag}(\bar{A})
\end{equation}
The graph structure $W$ is constructed as follows:
\begin{equation}
\begin{aligned}
   W &= \tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}\in \mathbb{R}^{T\times T}\\
\tilde{D} &= \mathrm{diag}(\sum_j^T\tilde{a}_{ij}) 
\end{aligned}
\label{eq:buildgraph}
\end{equation}
We believe that there is no need to design complex optimization objectives. By fixing the graph structure and iteratively optimizing prototypes and labels, excellent results can be obtained. We define the initial prototypes as:
\begin{equation}
\label{eq:originproto}
    C^0_n = \frac{1}{K}\sum_{\bar{\boldsymbol{x}}_i\in \mathcal{S}_n}\bar{\boldsymbol{x}}^s_i
\end{equation}
Subsequently, we obtain the label matrix $Z=[Z_s,Z_q]\in \mathbb{R}^{T\times K}$ as follows,
\begin{align}
\label{eq:supportlabel}
    Z_{s(in)} &= \mathrm{OneHot}(y_i^s)= \begin{cases}
 1 & \mathrm{ if }\ y_i^s= n\\
 0 & \mathrm{otherwise}
\end{cases} \in \mathbb{R}^{NK\times N}\\
\label{eq:querylabel}
    Z_{q(in)} &= \frac{\mathrm{exp}(-\lambda\|\bar{\boldsymbol{x}}_i^q-
    \bar{\boldsymbol{c}}^t_n\|^2_2)}{\sum_n^N \mathrm{exp}(-\lambda\|\bar{\boldsymbol{x}}_i^q-
    \bar{\boldsymbol{c}}^t_n\|^2_2)} \in \mathbb{R}^{M\times N}
\end{align}
We perform label propagatiosn based on the label matrix and solve the propagation results using a closed-form solution:
\begin{equation}
\label{eq:propagation}
    Z^t= (I-\alpha W)^{-1}Z
\end{equation}
where, $Z^t$ represents the label matrix after $t$ iterations, and $\alpha\in [0,1)$ is the scaling factor for label propagation. Compare to the traditional label propagation methods that solely relying on the labels of support samples, i.e., $Z=[\mathrm{OneHot}(y_i^s),\boldsymbol{0}_{M}]$, our method utilizes all samples as the source for label propagation, resulting in more accurate and robust results. Subsequently, we normalize the label matrix:
\begin{equation}
\label{eq:normalize}
    Z_{q}^t =\frac{z_{in}}{\sum_n^Nz_{in}} \quad i\in NK+1,\cdots T
\end{equation}
The labels for support samples $Z_s$ are normalized by Eq.\ref{eq:supportlabel}, and the labels for query samples $Z_q$ are normalized using Eq.\ref{eq:normalize}. We update prototypes based on the normalized label matrix $Z^t$:
\begin{equation}
\label{eq:updateproto}
C^t = (1-\beta) C^{t-1} + \beta (Z^t)^\top\bar{X}
\end{equation}
where, $\beta$ controls the update speed of prototypes. We iterate from Eq.\ref{eq:supportlabel} to Eq.\ref{eq:updateproto} for $n_{step}$ times, and based on the final label matrix $Z^{n_{step}}_q$, we predict the labels $y_i^q$ for the query set $\mathcal{Q}$ by:
\begin{equation}
\label{eq:predict}
    y_i^q = \mathrm{arg}\max_N(z_{in}^{n_{step}})\quad i\in NK+1,\cdots T
\end{equation}
The overall procedure is outlined in Algorithm 1. Through the aforementioned iterations, FILP effectively addresses several issues with existing label propagation methods. First, class prototypes and label propagation results can be iteratively optimized. Second, when the support sample distribution is biased, prototypes adaptively correct themselves based on the internal similarity of query samples. Third, when the number of query samples for each class is imbalanced, according to Eq.\ref{eq:propagation}, each query sample propagates its own label. Hence, the propagation strength for each class can adaptively adjust based on the number of query samples. Lastly, our method only needs to optimize prototypes and the label matrix that typically converges after 5 to 10 iterations, achieving better end-to-end real-time deployment performance.


\begin{algorithm}
\caption{Fast Iterative Label Propagation} 
\SetCommentSty{text}
\KwIn{Features $X=[\boldsymbol{x}_{1}^s,..,\boldsymbol{x}_{NK}^s,..{\boldsymbol{x}_{NK+M}^q}]^\top$, Support Labels $Y=[y_1^s,\cdots,y_{NK}^s]$, Hyperparamters $k,v,\alpha,\beta$}
\KwOut{Query Labels $y_i^q$}
$\bar{X} \leftarrow G'X = (I-\frac{1}{2}L)^kX$ \tcp*[r]{Eq.\ref{eq:featureprojectK}}

$W = \textsc{BuildGraph}(\bar{X},v)$ \tcp*[r]{Eq.\ref{eq:sparselink}, \ref{eq:diag}, \ref{eq:buildgraph}}
    $C^0_n = \frac{1}{K}\sum_{\bar{\boldsymbol{x}}_i\in \mathcal{S}_n}\bar{\boldsymbol{x}}^s_i$ \tcp*[r]{Eq.\ref{eq:originproto}}
$P = (I-\alpha W)^{-1}$\tcp*[r]{Speed Up Calculation}
\For{$t=1:n_{step}$}{
    $Z \leftarrow \textsc{Assign}(\bar{X},C^{t-1},Y)$\tcp*[r]{Eq.\ref{eq:supportlabel}, \ref{eq:querylabel}}
    $Z^t \leftarrow (1-\alpha)PZ$ \tcp*[r]{Eq.  \ref{eq:propagation}}
    $Z^t \leftarrow \textsc{Normalize}(Z,Y)$\tcp*[r]{Eq.\ref{eq:supportlabel},\ref{eq:normalize}}
    $C^t \leftarrow (1-\beta) C^{t-1} + \beta (Z^t)^\top\bar{X}$ \tcp*[r]{Eq.\ref{eq:updateproto}}
}
\KwRet{$y_i^q = \mathrm{arg}\max_N(z_{in}^{n_{step}})$}\tcp*[r]{Eq.\ref{eq:predict}}
\label{alg1}
\end{algorithm}

\subsection{Computational Analysis}
%The computational complexity of our proposed method is primarily dependent on the number of samples $T$ and the feature dimension $d$. 
Under the transductive few-shot learning scenario, both number of samples $T$ and feature dimension $d$ are typically small. The complexity of MGC for feature mapping is $O(T^2d)$, which can be considered negligible. During the FILP phase, to reduce the complexity of the matrix inversion operation in Eq.\ref{eq:propagation} as $O(T^3)$, we have adopted two optimizations into our approach: 1) the matrix is sparse, benefiting from the optimized solving speed of the LU decomposition algorithm, 2) as the graph is fixed, the propagation matrix $P = (I-\alpha W)^{-1}$ in Eq.\ref{eq:propagation} can be computed outside the iteration, as mentioned in Algorithm 1.
Thus, the overall complexity of our proposed method keep low. 
% Additionally, with only a few iterations needed, our method is several times faster than the current state-of-the-art methods and It can efficiently perform inference on CPUs.
